Polarized User and Topic Tracking in Twitter

Digital traces of conversations in micro-blogging platforms and OSNs provide information about user opinion with a high degree of resolution. These information sources can be exploited to under- stand and monitor collective behaviors. In this work, we focus on polarization classes, i.e., those topics that require the user to side exclusively with one position. The proposed method provides an iterative classification of users and keywords: first, polarized users are identified, then polarized keywords are discovered by monitoring the activities of previously classified users. This method thus allows tracking users and topics over time. We report several experiments conducted on two Twitter datasets during political election time-frames. We measure the user classification accuracy on a golden set of users, and analyze the relevance of the extracted keywords for the ongoing political discussion.

==> alg.tex <==
%!TEX root = main.tex
%\section{Models and Methods}


%\todo{Per le europee si puo' inserire una sezione di analisi del dataset. Sono stati suddivisi manualmente gli hashtag piu' frequenti (i primi 100) assegnando quelli piu' polarizzati per un partito a quel partito. Sono stati classificati gli utenti che usano prevalentemente gli hashtag polarizzati di un partito come votanti di quel partito. Sono stati creati i grafi delle cooccorenze a partire dagli hashtag polarizzati per partito considerando i tweet degli utenti classificati. Analisi delle metriche di rete che non mostrano grandi differenze tra le reti.}
\note{Network analysis and metrics calculated on the graph built considering the co-occurrences of hashtags in tweets written by polarized users do not show significant differences among classes, neither a specific behavior}.

\subsection{Evaluation methodology}

We built an evaluation dataset by identifying those users whose opinion can be
inferred with high confidence. During elections, as for other events, very
specific hashtags are used over Twitter to express a strong intention of vote.
We assume that users that frequently use one of such hashtags are strongly
sided with one of the competing parties and they will not change idea in the
short term. Such strong hashtags were handpicked among the 500 most frequent
in the data. \inote{specific hashtags? other name?} As reported in
Table~\ref{tab:hashtags}, those specific hashtags are of the kind {\tt \#i
-vote-party} for the \dataeu dataset, and puns for \datapd.\footnote{For the
sake of clarity, hashtags were always translated in English.}


\begin{table}
\centering
\caption{\label{tab:hashtags} Specific and Generic Hashtags.}
\begin{tabular}{lcc}
\hline
\multicolumn{3}{c}{{\bf Dataset: \datapd}} \\
Cand. & Generic Hashtags & Specific Hashtags \\
\hline
A 		& {\tt \#renzi}		& {\tt \#preferenzi}		\\
B 	& {\tt \#cuperlo}	& {\tt \#bettercuperlo}		\\
C 		& {\tt \#civati}	& {\tt \#voteus}			\\
\hline
\hline
\multicolumn{3}{c}{{\bf Dataset: \dataeu}} \\
Party & Generic Hashtags & Specific Hashtags \\
\hline
PD 			& {\tt \#pd}			& {\tt \#ivotepd}						\\
M5S			& {\tt \#m5s}			& {\tt \#ivotem5s}						\\
FI			& {\tt \#forzaitalia}	& {\tt \#votefi} {\tt \#voteitaly}		\\
LEGA		& {\tt \#lega}			& {\tt \#ivotelega} {\tt \#legathistime}	\\
AET			& {\tt \#tsipras}		& {\tt \#ivotetsipras} 					\\
\hline
\end{tabular}
\end{table}


The set of reference users were identified by applying Algorithm~\ref{alg:users-class} 
with the above hashtags as input. This guarantees that a user is
safely considered as {\em polarized} to a party $c \in \topics$ if its tweets
classified with $c$ are at least twice more frequent than any other class.
We denote with $\cusers=\{z_1, z_2, \ldots \}$ this set of polarized users,
and with $Z_c\subseteq \cusers$ those supporting a specific formation. 

The composition of the set \cusers is reported in
Table~\ref{tab:controlgroup}. The number of users is about 1,000 for both
datasets under consideration.  The control group is thus a small fraction of
the full dataset, which accounts for \inote{XXX users}. This is very
interesting, as it suggests that a global analysis  of the Twitter stream
cannot be based on a few trivial hashtags. Note that the relative popularity
of the parties is not proportional to the number of votes received, but it is
rather depending on the efficacy of the hashtag promoted.


\begin{table}
\centering
\caption{\label{tab:controlgroup} Composition of the control group. \inote{possiamo mettere anche il numero di tweets corrispondenti per non far sembrare troppo piccolo control group?}}
\begin{tabular}{lll|lll}
\hline
\multicolumn{3}{c|}{\datapd} &  \multicolumn{3}{c}{\dataeu} \\
 & Polarized & Polarized & & Polarized & Polarized \\
Cand. & Tweets & Users & Party & Tweets &  Users\\

\hline
\hline
A 		& 330 & 109	& PD 		& 262 & 129 	\\
B 	& 4759 & 243 		& M5S 		& 146 & 95 	 \\
C 		& 2925 & 700 	& FI 		& 1263 & 199 	 \\
	 		 & 	 	& 			& LN 		& 480 & 226  \\
			 &		&			& AET 	& 757 & 328 	\\ \hline
{\it total}	& 8014 & 1052				& {\it total}	& 2908 & 977  \\
\end{tabular}
\end{table}\

%\begin{tabular}{llrl|llrl}
%\hline
%\multicolumn{4}{c|}{\datapd} &  \multicolumn{4}{c}{\dataeu} \\
% & Polarized & \multicolumn{2}{c|}{Polarized} & & Polarized & \multicolumn{2}{c}{Polarized} \\
%Cand. & Tweets & \multicolumn{2}{c|}{Users} & Party & Tweets &  \multicolumn{2}{c}{Users} \\
%
%\hline
%\hline
%A 		& 330 & 109 	&(10\%)	& PD 		& 262 & 129 	&(13\%) \\
%B 	& 4759 & 243 	&(23\%)	& M5S 		& 146 & 95 	&(10\%) \\
%C 		& 2925 & 700 	&(67\%)	& FI 		& 1263 & 199 	&(20\%) \\
%	 		& & 	 	& 			& LN 		& 480 & 226 	&(23\%) \\
%			& &		&			& AET 	& 757 & 328 	&(34\%) \\ \hline
%{\it total}	& 8014 & 1052	&			& {\it total}	& 2908 & 977 	& \\
%\end{tabular}
%\end{table}


The set of users \cusers, also called {\em control group}, is used to evaluate
the users classification accuracy of the proposed method. Given the users
classification $U_c$ provided by some given algorithm, precision, recall and
F-Measure are restricted to the set \cusers. Formally, for any given class
$c \in \topics$, precision and recall are defined as:
\begin{equation}\label{eq:precision}
P_c (U_c) =  \frac{ U_c \cap Z_c}{U_c \cap \cusers} \quad\quad
R_c (U_c) =  \frac{ U_c \cap Z_c}{Z_c}
\end{equation}

The F-measure $F_c$ is the harmonic means of $P_c$ and $R_c$.
In addition, as the proposed algorithm may not be able to classify all of the users in \cusers,
we report also the coverage $C$ for the set of classified users:
\begin{equation}
C(U)= \frac{ \left( \bigcup_{c \in \topics} U_c \right) \cap \cusers }{ \cusers }
\end{equation}

\todo{compute micro and macro f-measure precision recall...}



% To evaluate the method we consider a subset of users that explicitly mention
% in a tweet their vote intention through an hashtag. This group of users, that
% we call \textit{control group} is denoted by the set $\cusers=\{z_1, z_2,
% \ldots \}$, for which the vote intention is known with a significant level of
% confidence, assuming that if a person explicitly expresses a vote option this
% is a true information and he/she is quite convinced, so not frequently he/she
% will change idea in a short term.  We proceed as follows:


% We classified the user \cusers following the Algorithm~\ref{alg:users-class}
% considering $H_c$ the previously identified hashtags for each class $c$. In
% Tab.~\ref{tab:cgpd} and in Fig.~\ref{fig:pddatacg} we reported the size of the
% control group \cusers for the first dataset considered, whereas in
% Tab.~\ref{tab:cgeu} and in Fig.~ \ref{fig:eudatacg} the values refer to the
% second dataset used.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{cgPD.png}
%     \caption{Composition of control group for dataset 1}
%     \label{fig:pddatacg}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{cgEU.png}
%     \caption{Composition of control group for dataset 2}
%     \label{fig:eudatacg}
% \end{figure}



\subsection{Polarized Users Tracking}

In this section we evaluate the goodness of the proposed algorithm in
detecting and classifying polarized users. The \myalgo algorithm must be fed
with a set of {\em generic} hashtags. These set of hashtags should be very
cheap to be extracted and they should roughly identify the topics and users to
be further refined by the algorithm. We used the hashtags consisting in the
name of the candidate or party, as they were always present and sufficiently
adopted in our datasets. Those seed hashtags are reported in
Table~\ref{tab:hashtags}.

We use the $k$-means\cite{macqueen1967some} clustering algorithm as a
baseline. Each user $u$ is represented with a vector of 500 features,
corresponding to the 500 most frequent hashtags in the dataset. The user
feature vector stores the frequency \inote{not binary!} of an hashtag in the
stream of tweets $\tweets_u$ published by the user. We imposed the number of
the clusters $k$ equal to the number of classes and, to simulate the same
starting condition of our method, we built the initial centroids so as to
encode the {\em generic} hashtags in Table~\ref{tab:hashtags}. The centroid
for the class $c$ is a vector holding 1 in correspondence of the generic
hashtag and 0 otherwise. The result of the $k$-means baseline is thus a
clustering of users based on the {\em generic} tags provided. Note that the
algorithm classifies every user in the dataset. 

\todo{Add another baseline classifying users on the basis on the full stream,
as in \cite{coletto}?}


% Before proceeding with the iterations of the Algorithm~\ref{alg:iterative} we
% introduce another benchmarking method. We applied k-means clustering to
% compare the results with an alternative well-known method.     
% We impose the
% number of the clusters equal to the number of classes and to simulate the same
% starting conditions of our method we expressly indicate the centroids to the
% clustering algorithm using the initial labels (name of the class). 
% We used as
% features for the model the first 500 more frequently used hashtags for each
% class $c$. The centroids where vectors with 1 in the component which is
% related to the hashtag containing the name of the class.

\note{claudio fin qui.}

\todo{Lista degli esperimenti (ogni esperimento una tabella o una figura):

\begin{itemize}
\item kmeans
\item altra baseline \cite{coletto}?
\item \myalgo: F-measure al variare delle iterazioni
\item \myalgo: Precision Recall F-measure per classe con il numero massimo di iterazioni
\item \myalgo: sensitivity: F-measure al variare delle varie soglie tunate a mano
\item \myalgo: Day by day F-measure plot
\item \myalgo: discussion of global hashtags discovered
\item \myalgo: discussion of day-by-day hashtags discovered
\end{itemize}
}



We classified users according using the previous hashtags following the steps described in the Algorithm~\ref{alg:users-class}.
We used this classification as a baseline for the method assuming that the mention of the class name is a good driver to express the preference to that class. 
This assumption is supported by many works in literature (for instance in \cite{tumasjan2010predicting}) and in particular for dataset 1 we showed \cite{coletto} that the counting of candidate mentions is a good predictor for the electoral outcome.
This initial classification (step 0 of the first iteration of Algorithm~\ref{alg:iterative}) can be evaluated through our control group. Precision, recall and F-Measure are reported in Tab.~\ref{tab:partnamepd} for dataset 1 and in Tab.~\ref{tab:partname} for dataset 2. 
F-measure has been calculated as the harmonic mean of precision and recall. 

In Tab.~\ref{tab:partnamepd} and Tab.~\ref{tab:partname} we reported a coverage value.


\begin{table}
\center
\caption{\label{tab:partnamepd} Baseline method: performance - \pd.}
\begin{tabular}{cccc}
\hline
Party & Precision & Recall & F-measure \\ 
\hline\hline
\textit{Renzi} & 0.268 & 0.624 & 0.375 \\
\textit{Cuperlo} & 0.714 & 0.144 & 0.240 \\
\textit{Civati} & 0.981 & 0.299 & 0.458 \\
\textbf{TOT} &  &  & \textbf{0.358} \\
\hline\hline
\textbf{Coverage} &  &  & 0.49 \\
\hline
\end{tabular}
\end{table}

\begin{table}
\center
\caption{\label{tab:partname} Baseline method: performance - \eu.}
\begin{tabular}{cccc}
\hline
Party & Precision & Recall & F-measure \\ 
\hline\hline
\textit{PD} & 0.574 & 0.209 & 0.306 \\
\textit{M5S} & 0.296 & 0.747 & 0.424 \\
\textit{PDL} & 1.000 & 0.231 & 0.375 \\
\textit{LEGA} & 0.990 & 0.912 & 0.949 \\
\textit{TSIPRAS} & 1.000 & 0.348 & 0.516 \\
\textbf{TOT} &  &  & \textbf{0.514} \\
\hline\hline
\textbf{Coverage} &  &  & 0.67 \\
\hline
\end{tabular}
\end{table}



\subsection{Polarized User Tracking}

We applied than Algorithm~{alg:hashtags-class} to identify for each class $c$ a set of polarized hashtag from the initial labels (hashtag of the party/candidate). We completed the first run of the Algorithm~\ref{alg:iterative} and we used the obtained new hashtags to reiterate the process, reclassifying again the polarized users.
Results for the new iteration are reported in in Tab.~\ref{tab:met1pd} and Tab.~\ref{tab:met1}. We reported in brackets the baseline value (first classification) to facilitate the comparison. Overall we obtained an increase of 38\% on average in the F-measure (+57\% for dataset 1 and +19\% for dataset) with only one iteration of the proposed algorithm. We increased the coverage of 53\% for dataset 1 and of 6\% for dataset 2. 

\begin{table}
\center
\caption{\label{tab:met1pd} First iteration: performance - \pd.}
\begin{tabular}{cccc}
\hline
Party & Precision & Recall & F-measure \\ 
\hline\hline
\textit{Renzi} & {\color{PineGreen} 0.592} (0.268) & {\color{red} 0.532} (0.624) & {\color{PineGreen} 0.560} (0.375) \\
\textit{Cuperlo} & {\color{PineGreen} 0.976} (0.714) & {\color{PineGreen} 0.169} (0.144) & {\color{PineGreen} 0.288} (0.240) \\
\textit{Civati} & {\color{PineGreen} 0.870} (0.981) & {\color{PineGreen} 0.804} (0.299) & {\color{PineGreen} 0.836} (0.458) \\
\textbf{TOT} &  &  & {\color{PineGreen} \textbf{0.561}} (0.358) \\
\hline\hline
\textbf{Coverage} &  &  & 0.75 \\
\hline
\end{tabular}
\end{table}



\begin{table}
\center
\caption{\label{tab:met1} First iteration: performance - \eu.}
\begin{tabular}{cccc}
\hline
Party & Precision & Recall & F-measure \\ 
\hline\hline
\textit{PD} & {\color{PineGreen} 0.703} (0.574) & {\color{PineGreen} 0.403} (0.209) & {\color{PineGreen} 0.512} (0.306) \\
\textit{M5S} & {\color{PineGreen} 0.379} (0.296) & {\color{PineGreen} 0.811} (0.747) & {\color{PineGreen} 0.517} (0.424) \\
\textit{PDL} & {\color{red} 0.967} (1.000) & {\color{PineGreen} 0.437} (0.231) & {\color{PineGreen} 0.602} (0.375) \\
\textit{LEGA} & {\color{red} 0.977} (0.990) & {\color{PineGreen} 0.929} (0.912) & {\color{PineGreen} 0.952} (0.949) \\
\textit{TSIPRAS} & {\color{red} 0.981} (1.000) & {\color{red} 0.320} (0.348) & {\color{red} 0.483} (0.516) \\
\textbf{TOT} &  &  & {\color{PineGreen} \textbf{0.613}} (0.514) \\
\hline\hline
\textbf{Coverage} &  &  & 0.71 \\
\hline
\end{tabular}
\end{table}

Before proceeding with the iterations of the Algorithm~\ref{alg:iterative} we introduce another benchmark method. We applied k-means clustering to compare the results with an alternative well-known method.    
We impose the number of the clusters equal to the number of classes and to simulate the same starting conditions of our method we expressly indicate the centroids to the clustering algorithm using the initial labels (name of the class). We used as features for the model the first 500 more frequently used hashtags for each class $c$. The centroids where vectors with 1 in the component which is related to the hashtag containing the name of the class. 

\note{Do we need to explain k-means?}

The results of k-means approach are reported in Tab.~\ref{tab:met1pd} and Tab.~\ref{tab:met1}.
 

\begin{table}
\center
\caption{\label{tab:kmeanpd} K-means method performance - \pd.}
\begin{tabular}{cccc}
\hline
Party & Precision & Recall & F-measure \\ 
\hline\hline
\textit{Renzi} & 0.101 & 0.275 & 0.148 \\
\textit{Cuperlo} & 0.226 & 0.535 & 0.318 \\
\textit{Civati} & 0.672 & 0.173 & 0.275 \\
\textbf{TOT} &  &  & \textbf{0.247} \\
\hline\hline
\textbf{Coverage} &  &  & 1.00 \\
\hline
\end{tabular}
\end{table}



\begin{table}
\center
\caption{\label{tab:kmeaneuropee} K-means method performance - \eu.}
\begin{tabular}{cccc}
\hline
Party & Precision & Recall & F-measure \\ 
\hline\hline
\textit{PD} & 0.301 & 0.364 & 0.330 \\
\textit{M5S} & 0.390 & 0.874 & 0.539 \\
\textit{PDL} & 0.460 & 0.628 & 0.531 \\
\textit{LEGA} & 0.995 & 0.916 & 0.954 \\
\textit{TSIPRAS} & 1.000 & 0.390 & 0.561 \\
\textbf{TOT} &  &  & \textbf{0.583} \\
\hline\hline
\textbf{Coverage} &  &  & 1.00 \\
\hline
\end{tabular}
\end{table}

K-means method performances are under the baseline for dataset 1 and for dataset 2 they stay in between our baseline and the results of the first iteration. To understand these results we have to consider that k-means create a partition of the users, labeling the entire set of users (coverage equal to 100\%), whereas the proposed method is more robust in the sense that it classifies only user which are highly polarized, keeping the users not easily polarized unlabeled (which could be people not lined up with one specific class).

\note{Descrizione del metodo con iterazioni e tabella con i risultati che mostrano la convergenza. Rispetto al caso con una sola iterazione si e' proceduto andando a fare l'update della classificazione ad ogni passo invece di ricrearla ogni volta.}


\subsection{Topic Tracking}

\note{Mostrare alcuni hashtag individuati dal metodo e gli scores.}

\subsection{Time evolution}

\note{Terrei il metodo indipendente nei giorni, quello continuous update e quello con selezione di una parola diversa al giorno. Descrizione e risultati. Inoltre per uno dei metodi mostrerigli ht che trova e come cambiano giorno per giorno.}



%\item Classification of all tweets in relation to the extracted polarized hashtags in this way:

% \begin{algorithm}
% \label{alg:alg1}
%  \KwResult{Classification of the users giving a list of sets of polarized hash-tags $H_{group1}$,..,$H_{groupN}$}
%  \For{all tweets in the collection}{
%   \eIf{$H_{tweet} \cap H_{groupT} \ne \emptyset$ and for all other sets $H_{tweet} \cap H_{groupX} = \emptyset$ with $X \ne T$}{
%    mark the tweet with the name of the $groupT$\;
%    }{
%    do not mark the tweet\;
%   }  
%  }
%   \For{all users in the collection}{
%   count the number of marked tweets for each $H_{group}$ and sort descending these values $V$\\ 
%   \eIf{$V$ is unique or $V_{H_{group_{1st}}}>2*V_{H_{group_{2nd}}}$}{
%    mark the user with the name of the $group_{1st}$;
%    }{
%    do not mark the user\;
%   }  
%  }
%  \caption{Users classification algorithm}
% \end{algorithm}


%
%PRIMARIE
%
%renzi=['renzi']
%cuperlo=['cuperlo']
%civati=['civati']\\
%
%EUROPEE
%
%tsipras=['tsipras']
%lega=['lega']
%pdl=['forzaitalia']
%pd=['pd']
%m5s=['m5s']\\










\begin{table}
\center
\caption{\label{tab:metIterpd} Iterative Method: performance - PRIMARIE PD.}
\begin{tabular}{cccc}
\hline
Step & F-measure \\ 
\hline\hline
\textit{Step 1 (baseline method)} & 0.358 \\
\textit{Step 2 (method 2)} & 0.580\\
\textit{Step 3} & 0.597\\
\textit{Step 4} & \textbf{0.599}\\
\hline\hline
\textbf{Coverage} & \textbf{0.88} \\
\hline
\end{tabular}
\end{table}

\inote{Results of stage 2 of the iterative method are slightly different from method 2 because in this implementation the the classification is in update of the previous step and not independent.}


We tried
different alternative filtering approaches and it turned out that the selected
network metrics (with the respective values) give better results. In
Tab.~\ref{tab:met1alt} we reported some of the results of the 1-step iteration
algorithm applying different filtering approaches: in particular we show the
results skipping the filtering step, with the filtering step and applying a
post filtering, limiting the number of discovered hashtags to n (n=20) or
changing the threshold (from 0.001 to 0.003) on the score $S$ described in the
following paragraphs, which is a metric of the goodness of an hashtag for a
specific class. \inote{CLA: gli exp nella parte sperimentale e non qui}






\begin{table}
\center
\caption{\label{tab:met1alt} 1-step method: alternatives - \eu.}
\begin{tabular}{cccc}
\hline
Method & F-measure \\ 
\hline\hline
\textit{Network filters} & 0.613\\
\textit{No network filters} & 0.599\\
\textit{High threshold} & 0.611\\
\textit{Top \textit{k} hashtags} & 0.362\\
\hline
\end{tabular}
\end{table}

\inote{In Table ''Method 2 alternative'' we report results of alternative methods, changing the threshold from 0.001 to 0.003, removing the filters based on the network (bet centr, ...), limiting the number of classified hashtags to 20.}

\begin{table}
\center
\caption{\label{tab:metIter} Iterative Method: performance - EUROPEAN.}
\begin{tabular}{cccc}
\hline
Step & F-measure \\ 
\hline\hline
\textit{Step 1 (baseline method)} & 0.514 \\
\textit{Step 2 (method 2)} & 0.626\\
\textit{Step 3} & 0.627\\
\textit{Step 4} & \textbf{0.627}\\
\hline\hline
\textbf{Coverage} & \textbf{0.82} \\
\hline
\end{tabular}
\end{table}

\begin{table}
\center
\caption{\label{tab:met1daily} Method day by day: performance - EUROPEAN.}
\begin{tabular}{cccc}
\hline
Method & F-measure (Method 2) \\ 
\hline\hline
\textit{INDEPENDENT - AVG} & 0.404 (0.319)\\
\textit{ADDITIVE - LAST DAY} & \textbf{0.626} (0.573)\\
\textit{CONTINUOUS UPDATING - LAST} & \textbf{0.626}\\
\textit{ITERATIVE (1 ht) - LAST} & 0.615\\
\textit{ITERATIVE - LAST} & 0.508\\
\hline
\end{tabular}
\end{table}

\inote{In Table ''Method 2 day by day'' we report results of the procedure iterating day by day. The INDEPENDENT method refers to the method 2 applied every day starting from the hashtags with the name of the parties (results are an average on the considered days) The result in parentheses is the averaged baseline method. The ADDITIVE method differs from the previous one because the classification in each day is an update of the results of the previous days (considering separately method 2 and baseline method). In CONTINUOUS UPDATING METHOD the results at each step are an update. For instance, the baseline method of day 2 updates the result of method 2 in the first day and method 2 of day 2 updates the baseline results for that day. ITERATIVE method is similar to the previous one with the only difference that the starting hashtags each day are not always the party names hashtags by default, ma the most frequent hashtag among the classified ones in the previous step the day before. Last iterative method consider the iterative procedure day by day starting every day with the set of hashtag discovered in the previous day (It is the same procedure applied to total data in the iterative procedure, but in this case it doesn't work very well because it doesn't consider much the new hashtag od that day).}

%
%
%\begin{itemize}
%\item Method 2: We use the classification of Method 1 to built a graph for each political party of the co-occurrences of hashtags in the tweets whose users are marked with the party name according to the classification process described before. We limit the number of hashtags of each party to 500. 
%
%
%\item For each party we consider the nodes of the relative co-occurrence network according to the following criteria:
%degree ($>1$), closeness($>0.1$) and betweeness centrality ($>0$)
%\item For each party $p$ we will have a list of discovered hashtags $H_p$. 
%
%
%\item For each hashtag $h$ we calculate the Jaccard Index in this way:
%\begin{equation}\label{eq:normalize}
%\nonumber JaccardIndex_p(h) = J_p(h)= \frac{\phi(h,p)}{\phi(h)+\phi(p)-\phi(h,p)} 
%\end{equation}
%with $\phi(h,p)$ equal to the number of tweets containing at the same time the hashtags $h$ and $p$ (name of the party).
%
%\item For each $h$ in $H_P$ we calculate the score $S_p(h)$
%\begin{equation}\label{eq:normalize}
%\nonumber Score_p(h) = S_p(h)= J_p(h)\times\prod_{\bar{p} \in P-\{p\}}(1-J_{\bar{p}}(h))
%\end{equation}
%
%\item I exclusively assign $h$ to a party $p$ if $S_p(h)$ is greater than $\sigma$ with $\sigma = 0.001$ and if the score for other parties $S_{\bar{p}(h)}$ is less than $S_p(h)$. The procedure is summarized in algorithm~\ref{alg:alg2}.

% \begin{algorithm}
% \label{alg:alg2}
%  \KwResult{Classification of the polarized hash-tags}
%  \For{each party $p$ in $P$}{\For{each hash-tag $h$ associated to the party $p$}{
%   \eIf{$S_p(h)>\sigma$ and $S_p(h)>S_{\bar{p}}(h)$ for all $\bar{p} \ne p \in P$}{
%    assign the hash-tag $h$ to the $H_p$ set
%    }{
%    do not assign it\;
%   }  
%  }
%  }
%  \caption{Hash-tag discrimination algorithm}
% \end{algorithm}
%
%
%\item We then classify tweets and users with algorithm~\ref{alg:alg1} using as $H_p$ the new sets of hashtags identified with the method

%\item Calculation of F-measure, recall and precision.
%Results are in Table \ref{tab:met1}.



The objective of the work is:

\begin{itemize}

\item visualize iteratively the network of the hashtags relevant for the electors of a party

\item topic identification starting from the party name/ candidate name

\item optimized reiterative model (modeling)

\item debiasing (evaluate the bias of twitter users)

\end{itemize}
Other interesting information on the dataset. See Table\ref{tab:info} and \ref{tab:info2}
\\
\begin{table}
\center
\caption{\label{tab:infopd} Data Analysis - \pd}
\begin{tabular}{cccc}
\hline
Users & Averaged Number of tweets per user \\ 
\hline\hline
\textit{All data set} & 5.50\\
\textit{Control Group} & 31.14\\
\textit{Method 1} & 11.75\\
\textit{Method 2} & 6.81\\
\hline
\end{tabular}
\end{table}

\begin{table}
\center
\caption{\label{tab:info} Data Analysis - \eu}
\begin{tabular}{cccc}
\hline
Users & Averaged Number of tweets per user \\ 
\hline\hline
\textit{All data set} & 7.16\\
\textit{Control Group} & 71.21\\
\textit{Method 1} & 22.85\\
\textit{Method 2} & 14.23\\
\hline
\end{tabular}
\end{table}

Futuro:
\begin{itemize}

\item machine learning per il modello

\item non solo hashtag ma parole

\item sentiment

\item altri grafi (retweet, menzioni)

\end{itemize}



==> related.tex <==
%!TEX root = main.tex
\section{Related Work}
\label{sec:related}

In the recent years, the analysis of blogging platforms and streaming
information sources (e.g. Twitter) has received great attention in the Information Retrieval
and in the Data Mining communities. The present work is related to the
Topic Detection and Tracking (TDT) subject \cite{allan2012topic}, which has been
widely explored within the scope of news stream analysis \cite{walls1999topic}. 
In particular we focus on content and user tracking for polarized users. This notion is connected with the concept of controversy in Social Media, which have been studied, mostly in political contexts, using data coming from different sources (blogs \cite{adamic2005political}, Twitter \cite{conover2011political}, Facebook\cite{bessi2014social}, news  \cite{mejova2014controversy}).
Moreover another related research area is that of trending topics analysis. 
A trend detection mechanism is proposed in
\cite{mathioudakis2010twittermonitor}, where bursty keywords are detected and
then merged into groups on the basis of their co-occurrence. Finally, matrix
factorization and entity extraction methods are employed to find a few
representatives for each group. In \cite{cataldi2010emerging} trendiness is defined
on the basis of the user authority and of
the newly introduced keyword aging model which estimates the {\em energy} of a
term over time, providing only a qualitative evaluation.
The authors of \cite{lin2011smoothing} use a language model based approach to
attack the TDT problem specifically on Twitter data. They proposed to build a
foreground and a background language model, respectively capturing recent
past tweets, and different smoothing techniques are evaluated. Each topic is
identified by a hashtag. Similarly,
in \cite{yang2014large} a classification algorithm of tweets is proposed by mean of a hierarchy of topical categories. Training data is built
by exploiting web page links in tweets, and only textual features are
exploited. 
%The resulting classifier is then used to detect relevant topics for
%authors of tweets and for mentioned hashtags.
%
Our approach is different in several regards from current literature and it is not aimed at classifying the topic of discussion of a given
tweet or at detecting trending topics. We rather focus on the
identification of polarized communities.
% users. Such users classification is then
% used to discover relevant hashtags for each polarized class. Such
% identification of users and hashtags is boosted through a virtuous cycle able
% to detect the most correlated hashtags to each given polarized class. In
% addition, the framework allows the monitoring of the communities of polarized users
% and of their discussions over time.

Some approaches based on networks analysis have been proposed to study polarization of users in social networks. For instance, in \cite{conover2011political} the authors studied the network of retweets and mentions to analyze the segregation of users using different clustering approaches. Recently \cite{garimella2015quantifying} Garimella et al. proposed a graph-based method to identify controversy regarding topics by analyzing properties of the partitioned graph of social interactions.
In our case we want to study the polarization from a topical point of view.
% , proposing a methodology to label the conversations in time and to classify polarized users with an iterative approach alternative to network clustering, which will be used as a baseline.   

For our experiments we used Twitter data related to political events. 
% Our approach is based on the classification of users which polarize on a single category: for this reason the political tweets are a suitable example. 
Several works have tried to predict election results by analyzing data
from on-line social networks. Some of them have found that the counts of
tweets or users mentioning a political party is highly correlated with final
electoral results \cite{tumasjan2010predicting,digrazia2013more}.
Those counts can be improved with content and sentiment analysis
\cite{bermingham2011using,coletto}. In this work we aim to track users polarization and topics of the discussion in order not to forecast political events, which is a task highly exploited and undermined by difficulties (user bias, data dependency), but to monitor the {\em polarized} communities and their topics in the given data stream.
% We use electoral data to conduct our experiments, but the
% proposed algorithm is usable to several application fields. 
% The task is challenging and the evaluation of the methods implies a quantitative analysis and a qualitative one. 
Finally, we propose an evaluation methodology.
 % and in addition to that we discuss the results under a qualitative perspective. 
% \note{Debiasing}
% Twitter profiles do not include demographic information (sex, age, etc.). For this reason dealing with the bias issue is tricky. A few works applied debiasing techniques. In \cite{gayo2011don} Gayo-Avello operates a debiasing procedure assigning the age to a sample of data by crossing names with online public records. \cite{Sang} tries a different approach, debiasing the data according to the presumed political leaning of the population. In both cases the methods, even though they reduce the prediction error, are partial and they rely on external data, lacking of accuracy.
